Enhancement of High-definition Map Update Service Through Coverage-aware and Reinforcement Learning

High-definition (HD) Map systems will play a pivotal role in advancing autonomous driving to a higher level, thanks to the significant improvement over traditional two-dimensional (2D) maps. Creating an HD Map requires a huge amount of on-road and off-road data. Typically, these raw datasets are collected and uploaded to cloud-based HD map service providers through vehicular networks. Nevertheless, there are challenges in transmitting the raw data over vehicular wireless channels due to the dynamic topology. As the number of vehicles increases, there is a detrimental impact on service quality, which acts as a barrier to a real-time HD Map system for collaborative driving in Autonomous Vehicles (AV). In this paper, to overcome network congestion, a Q-learning coverage-time-awareness algorithm is presented to optimize the quality of service for vehicular networks and HD map updates. The algorithm is evaluated in an environment that imitates a dynamic scenario where vehicles enter and leave. Results showed an improvement in latency for HD map data of $75\%$, $73\%$, and $10\%$ compared with IEEE802.11p without Quality of Service (QoS), IEEE802.11 with QoS, and IEEE802.11p with new access category (AC) for HD map, respectively.

==> abbrv.tex <==
% Normal table (single column)
\begin{table}
    \caption{Abbreviation Table}
    \centering
    \begin{tabular}{c|c}
    \hline
    Abbreviation & Definition \\
    \hline
    5GAA & 5G Automotive Association \\
    AC & Access Category \\
    AIFSN & Arbitration Inter-Frame Space Number \\
    AV & Autonomous Vehicles \\
    CDF & Cumulative Distribution Function \\
    CPU & Central Processing Unit \\
    CW & Contention Window \\
    DQN & Depp Q Network \\
    EDCA & Enhanced Distributed Channel Access \\
    HD Map & High Definition Map \\
    LSTM & Long Short-term Memory \\
    MAC & Media Access Control \\
    ML & Machine Learning \\
    ms & Millisecond \\
    QoS & Quality of Service \\
    RSU & Radio Station Unit \\
    SAE & Society of Automotive Engineers \\
    slope & Slope for Direction \\
    VANET & Vehicular Ad-hoc Network \\
    VRU & Vulnerable Road User \\
    \end{tabular}
    \label{tab:abbrevation}
    \end{table}
    
